ModuleGuard:Understanding and Detecting Module Conflicts in Python Ecosystem

Python has become one of the most popular programming languages for software development due to its simplicity, readability, and versatility. As the Python ecosystem grows, developers face increasing challenges in avoiding module conflicts, which occur when different packages have the same namespace modules. Unfortunately, existing work has neither investigated the module conflict comprehensively nor provided tools to detect the conflict. Therefore, this paper systematically investigates the module conflict problem and its impact on the Python ecosystem. We propose a novel technique called InstSimulator, which leverages semantics and installation simulation to achieve accurate and efficient module extraction. Based on this, we implement a tool called ModuleGuard to detect module conflicts for the Python ecosystem. For the study, we first collect 97 MC issues, classify the characteristics and causes of these MC issues, summarize three different conflict patterns, and analyze their potential threats. Then, we conducted a large-scale analysis of the whole PyPI ecosystem (4.2 million packages) and GitHub popular projects (3,711 projects) to detect each MC pattern and analyze their potential impact. We discovered that module conflicts still impact numerous TPLs and GitHub projects. This is primarily due to developers' lack of understanding of the modules within their direct dependencies, not to mention the modules of the transitive dependencies. Our work reveals Python's shortcomings in handling naming conflicts and provides a tool and guidelines for developers to detect conflicts.

==> backups/New_study.tex <==
\section{Large scale study}
This section we introduce the design of the large scale study and answer to the RQs.

\subsection{RQ1: conflict between module names and package names}
\textbf{Design.} \loancold{This is not design.} To answer RQ1, we select 3.91 million projects from PyPI, and analysis their direct dependencies and module paths with our technique proposed in \cref{chapt:tech1} and \cref{chapt:tech2}. For each module path, we translate it to the module name that can be imported. If there is no module with the same package name among the modules that can be imported, we assume that there is a conflict between module name and package name.
\textbf{Impact.} As we discuss in \cref{motivation}, module names can easily be misused as package names to install, resulting in typosquatting attacks. As an interpreted language, python projects are distributed with installation scripts that allow developers to execute code. Attackers use social engineering or typosquatting to make the developer download malicious packages, execute malicious scripts during pip installation, then read critical files in the system and send them to the attackers. But this type of attack by installing scripts is easy to detect. In fact, python runs the code in the module when it is imported. If the attack is launched while the python code is running instead of at installation time, it can greatly reduce the probability of being detected. 

So a complete attack chain could look like this, where an attacker could write malicious code in the module's \_\_init\_\_.py file and upload it as a package with the same name. At the same time this package name is the module name of another popular package, which can easily be downloaded by developers by mistake. Nothing happens when the developer downloads the malicious package, and he thinks he has downloaded the right package to fix the error reported by python. However, when he runs the statement that imports the corresponding module in the python code through the python interpreter, python will automatically run the malicious code in \_\_init\_\.py, at which point the attack has been completed without the developer noticing. Even the attacker can add the correct function logic to the malicious code, so that python will not report any error even if the code finishes running. \loancold{Why does this paragraph of "attack chain" appear in the large scale study section?}

\textbf{large scale statistic.} 
We found a total of 1093,012 projects have module conflict with their package name on PyPI, accounting for 28\% of the entire ecosystem. What's worse, most of these projects do not have a corresponding honeypot project created on PyPI, leading to the possibility that most of these packages could be affected by the previously mentioned attack. So we recommend developers to make the module name of their project consistent with the project name before uploading to PyPI. \loancold{Add table/figure and findings of results in different dimension.}

\subsection{RQ2: conflict between packages and its dependencie}
\textbf{Design.} To answer RQ2, we select 3.91 million projects from PyPI, and build their dependency graphs using resolvlib\cite{resolvelib}. Based on the generated dependency graph, we follow the dependency graph to find if there are module path conflicts between all the dependencies. If there is a conflict in the module path between the dependencies of a project, we consider the project to have a pattern B conflict.

\begin{figure}
\centering
    \begin{subfigure}[b]{0.45\textwidth}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
pkg1-0.0.1
--sub.py
--mod1
----__init__.py
----add.py
\end{minted}
\caption{pkg1 module structure}
\label{example: pkg1 module structure}
\end{subfigure}

\centering
\begin{subfigure}[b]{0.45\textwidth}
\vspace{10pt}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
pkg2-0.0.1
--sub.py
--mod1
----__init__.py
----mult.py
\end{minted}
\caption{pkg2 module structure}  
\end{subfigure}%
\label{example: pkg2 module structure}

\centering
\begin{subfigure}[b]{0.45\textwidth}
\vspace{10pt}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
site-packages
--sub.py(overwirte)
--mod1
----__init__.py(overwirte)
----mult.py
----add.py
\end{minted}
\caption{after install pkg1 and pkg2}  
\end{subfigure}%
\label{example: after install pkg1 and pkg2}

\caption{Pattern B example}
\label{example: Pattern B example}
\vspace{-16pt}
\end{figure}

\textbf{Impact.} In contrast to Pattern A, we further found that when two projects have the same module path, overwriting occurs when both projects are installed in one environment. Since pip installs all modules in the same environment into the site-package folder, and there is no separate folder for each installed project to distinguish between them, resulting in if two projects have the same files, the latter will overwrite the former's files. \cref{example:Pattern B example} gives a simple example of Pattern B conflict. Suppose pkg1 and pkg2 are two dependencies of a project. As \cref{example: pkg1 module structure} shows, the pkg1 has a sub module and a mod1 module, and the mod1 module has an add submodule. As \cref{example: pkg2 module structure} shows, the pkg2 has a sub module and a mod1 module, and the mod1 module has a mult submodule. Suppose we install pkg1 first and then pkg2. After installation pkg1 and pkg2 are mingled in the site-package folder. The sub.py and mod1.\_init\_\.py of pkg2 will overwrite pkg1, and mod1 has two submodules, mult and add. To make matters worse, pip does not report a warning about the override after the installation is complete. If the malicious code is present in the post-installed package and overwrites the normal code files in the local environment, the developer will invoke the malicious code unconsciously after importing the modules that have been corrupted. (\loancold{Paragpragh too long.})
So the complete attack chain could look like this: the attacker finds a popular project and carefully constructs a package with the same module path to upload. The attacker then uses social engineering to corrupt the dependencies of popular projects or otherwise cause developers to download the malicious package and silently overwrite the relevant path in the developer's local environment. Or there are module conflicts in different dependencies of popular projects, and some modules have been overwritten when the project is pip installed. When the module is subsequently used on this machine, the code in the malicious module will be imported and executed, and the local secret files will be read. \loancold{Why does this paragraph of "attack chain" appear in the large scale study section? If the pattern of the attack is one of your results, raise a separate RQ of MC attack pattern.}

\textbf{large scale statistic.}
We find 163,552 projects out of a total of 3.91 million projects on PyPI, which had module conflicts between its dependencies. Although the package with MC only occupies 4.71\% of the whole ecosystem, it contains some projects of internet giant companies such as google, Microsoft, Amazon and so on. Worse still, some projects overwrite even more than 100 paths, with a large attack surface. This type of attack is stealthy and  more difficult to detect.

==> backups/background_and_motivation.tex <==
% terminology:
% Here we first clarify some definitions based on the official python documentation\cite{pydocumentation}, and the terminology in the subsequent paper will follow these definition criteria.

% \textbf{project:} This terminology in this paper is referenced from the PyPI official website\cite{pypi}. A projects is a unique identifier for packages on PyPI that includes all releases of the packages. The name of a project is also called package name. As of November 2022, there are more than 400,000 projects on PyPI.

% \textbf{release:} This terminology in this paper is referenced from the PyPI official website\cite{pypi}. A release refers to a specific version of a project. As of November 2022, there are more than 3.91 million releases on PyPI.

% \textbf{module:} This terminology in this paper is referenced from the python documentation\cite{pydocumentation}. A module is a file containing Python definitions and statements. The file name is the module name with the suffix .py appended.

% \textbf{package:} This terminology in this paper is referenced from the python documentation\cite{pydocumentation}. A package refers to a Python module which can contain submodules or recursively, subpackages. Packages also include Regular packages and namespace packages. Regular packages are those can be directly imported by others. If it is a directory, it requires the \_\_init\_\_.py file under the directory. Conversely, namespace packages omit \_\_init\_\_.py.

% rust那边背景介绍比较好写，因为RUF接触的人少，但是对于python而言背景介绍显得比较苍白，有什么办法解决不。 
\section{Background and motivation}

\loancold{You can write your design and implementation first. During the writing, you will find that you need to declare some important features, entities, and mechanisms first. These explanations are then written in this section. Right now, we can add as much needed detail as possible, after Alpha paper is constructed, we can reconsider this section, if needed.}

\xingyu{ Add Definition of Package Module}

In this section, We first introduce the background of how PyPI manage dependencies and the background of python dependency resolution. Then We describe two motivation examples.

% python dependency configure
\begin{figure}
\centering
    \begin{subfigure}[b]{0.45\textwidth}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
versioneer[toml]
cython==0.29.32
pytest>=6.0
pytest-cov
\end{minted}
\caption{requirement.txt}
\label{code:requirement.txt}
\end{subfigure}

\centering
\begin{subfigure}[b]{0.45\textwidth}
\vspace{10pt}
\begin{minted}[fontsize=\footnotesize, linenos]{python}
setup(
    name = "versioneer",
    version = "0.0.1",
    packages = find_packages(),
    install_requires = [
        "python-dateutil>=2.8.1",
        "pytz>=2020.1",
        "numpy (>=1.20.3) ; python_version < '3.10'",
        ],
    extras_require = {
        "toml": ["hypothesis>=5.5.3"],
    }
)
\end{minted}
\caption{setup.py}  
\end{subfigure}%

\label{code:setup}
\caption{dependency management}
\label{fig:dependency management}
\vspace{-16pt}
\end{figure}


  
\subsection{Python dependency management}
\label{Python dependency management}
Python uses pip (\loancold{It is a specific entity, highlight. Similar issues in this section should be taken care of.}) to manage its dependencies. Developers can write all project dependencies to the requirement.txt file and use "pip install requirement.txt" to install all dependencies. The format of requirement.txt is shown in \cref{code:requirement.txt}. Each of these lines represents a dependency. The "toml" in "\[\]" in the first line indicates the use of the extra dependency under the "toml" feature of the versioneer project.

Developers can also upload their projects to PyPI and share them with others. (\loancold{Give official reference and formally introduces them.})When uploading the project, the developer needs to write the dependency information to the "install\_require" and "extra\_require" field in the setup.py file, and use the setuptools\cite{setuptools} to compile the project into a source package or binary package for uploading. \cref{code:setup} is a simple example of a setup.py script. It contains three ordinary dependencies and one extra dependency. When the project is depended by someone else, pip will install its three common dependencies. But when a developer wants to enable the "toml" functionality, as in \cref{code:requirement.txt}, pip will also install the dependency "hypothesis>=5.5.3". 

\textbf{Source package.} Source package records the project's information in the egg-info folder, which includes its dependencies and metadata. Other developers will need to unpack it locally after downloading and then compiling it in order to use it. The suffixes of source packages usually are tar.gz, zip, etc.

\textbf{Binary package.} Binary package records the project's information in the dist-info folder. Its information format is different from source packages. The suffixes of binary packages usually are whl, egg, etc.
% Python does not have an official database of direct dependency information for all 3.91 million projects on PyPI. 
% Although some websites\cite{githubpipdb, watchman-web, Libio, depsdev} can provide direct dependency information for PyPI projects, these sites suffer from some disadvantages. Firstly, they do not record extra dependency information, resulting in inaccurate and incomplete dependency trees. Besides, some projects on PyPI are removed by maintainers, and most tools only consider incremental updates without considering the removed projects, which results in outdate datasets. What's more, some websites also set anti-crawl measures, which are not efficient for crawling 3.91 million projects. 

% On the other hand, pip\cite{pip}, the official package management for python, has a complex mechanism for extract dependency information. It first needs to download the projects locally, extract them to a temporary folder, and then run the setup.py file dynamically to get the dependency information. This approach will reduce efficiency due to dependency hell\cite{dependency-hell} and dependency conflict\cite{wang2020watchman} issues, although it is the most accurate way to obtain dependencies.

% As a result, a fast direct dependency extraction tool and a reliable dataset of directly dependent information is urgently needed. 

\subsection{Python dependency resolution}

Prior to version 20.3, pip used an older version of dependency resolution, which was deprecated due to inefficiencies and inability to handle dependency conflict issues. Since version 20.3, pip uses the dependency resolver that supports backtracking. Backtracking means that during dependency resolution, pip assumes a specific version as the candidate, and if that version does not match, pip backtracks to select another version and aborts the work done by the previous wrong path. This policy will increase the resolution time, but can effectively handle the dependency conflict issues. 

Fortunately, pip's resolution has now been separated into a project called resolvelib, and it has been uploaded to PyPI. Only a small number of interfaces need to be implemented to reproduce pip's backtracking resolution strategy.

\subsection{Motivation}
\label{motivation}

\xingyu{ Highlighting the security impact of MC behavior, BeautifulSoup is better example than opencv}
Our motivation example is opencv-python\cite{opencv} on PyPI. We find that we use "pip install opencv-python" to download it from PyPI. However, we use "import cv2" When using the project in code. This means that PyPI uses project name "opencv-python" to uniquely identify the package, and developers need to use the module name "cv2" when import it, which is not unique. 

Besides, if opencv-python is not installed on the developer's device, python will report the error "No module named "cv2"" when running codes that contains "import cv2". Some developers would use "pip install cv2" to fix the error report by mistake. Fortunately there is no project named cv2 on PyPI, so the developers would easy to find they make some mistakes.  (\loancold{Clearly illustrate how severe MC is, and how hard it is to fix this issue.}

So we find another example, a project named beautifulsoup4\cite{beautifulsoup4}. Its project name is "beautifulsoup4" and its module name is "bs4". Interestingly, there is a honeypot named the same name "bs4" on PyPI. This means that some project maintainers are already aware of the MC problem and have uploaded honeypot to prevent confusion attack. 

What's more, we did a lot of literature research and find that there is no work about a large scale study of MC issues on PyPI. As a result, we decided to do the new study and explore the possible attack surface and impact of the MC issues. \loancold{Not suitable for the writing.}


==> backups/direct_dependency_extraction.tex <==
\section{direct dependency extraction}
\label{chapt:tech1}
\xingyu{ 1. Direct Dependency information extraction 2. Dependency Resolution}

\loancold{1. The whole sections (3 and 4) looks like the introduction of a tool rather than your research method. You have to focus on the unique part of our research. 2. You should describe your method like a system. Every part of it has target functionality, and they operate together to solve the last big problem of your research target. Readers should know their connection, then they can think and feel that they have learnt from your paper. 3. Too much detail. We should try to avoid introduce file name "xxx.py"/"xxx.txt" and use defined name according to their functionality when explaining your design. 4. Explain one thing in one sentence. Each sentence should be strongly connected together. I'm totally lost in endless detail and loosely connected sentences, especially in 3.3.}

This section we introduce how we extract direct dependencies accurately and fastly using our novelty technique. 
\subsection{Challenge}
\label{difficulty1}
\loancold{To do sth, we need to extract direct dependencies. However,}
Python does not have an official database of direct dependency information for all 3.91 million projects on PyPI. 
Although some websites\cite{githubpipdb, watchman-web, Libio, depsdev} can provide direct dependency information for PyPI projects, these sites suffer from some disadvantages. Firstly, they do not record extra dependency information, resulting in inaccurate and incomplete dependency trees. Besides, some projects on PyPI are removed by maintainers, and most tools only consider incremental updates without considering the removed projects, which results in outdate datasets. What's more, some websites also set anti-crawl measures, which are not efficient for crawling 3.91 million projects. \loancold{Why it can't be directly solved? If can, it seems not so difficult. If can't, tell why and readers know that this is a difficult problem.}

On the other hand, pip\cite{pip}, the official package management for python, has a complex mechanism for extract dependency information. It first needs to download the projects locally, extract them to a temporary folder, and then run the setup.py file dynamically to get the dependency information or get it from metadata folder. This approach will reduce efficiency due to dependency hell\cite{dependency-hell} and dependency conflict\cite{wang2020watchman} issues, although it is the most accurate way to obtain dependencies.

Since there are various file format on pypi such as whl, egg, tar.gz, zip, etc., and the dependency definition is complex, it is complicated and difficult to obtain direct dependencies. Besides, every day there are many projects created and updated on PyPI. As a result, a fast direct dependency extraction tool and a reliable dataset of directly dependent information is urgently needed. 
 
\subsection{Daily updated local repository}
\xingyu{ This seems to be pure engineering work}

To conduct the large scale study, we first need to download all files from PyPI and extract direct dependency information. Here we use the bandersnatch\cite{bandersnatch}, an automated PyPI mirroring tool. We run it in a docker environment and start it automatically once a day, so that we get the latest information. But it has a drawback, like most of the state of the art tools\cite{Wang2022SmartPip, wang2020watchman, githubpipdb}, it only considers incremental updates and not the deleted projects. Excess project data can make dependency resolution inaccurate. For example, project A has two releases 1.0.0 and 1.1.0. the developers use pip to download the latest version 1.1.0. The maintainer then uploads the 1.2.0 release, but after being synchronized with the local mirror, maintainer removes it due to a bug in release 1.2.0. For a long time, the release 1.2.0 will be installed if using the local mirror, but the installation using pip was 1.1.0.

To solve this problem, We use the XMLRPC API of pypi.org. Its changelog\_since\_serial API is able to log all event changes on PyPI, including adding releases, adding files, deleting releases, etc. Each day before synchronization we record an event serial number. and process all events between that serial number and the last recorded serial number. When we find a delete event we remove the project file from the local mirror accordingly.


\subsection{multidimensional dependency extraction}
In \cref{Python dependency management} and in \cref{difficulty1} we introduce how python declare dependencies and difficulty of extracting direct dependency from project files. To solve this challenge, we propose the multidimensional dependency extraction technique, which obtains direct dependency information from PyPI API, metadata information and configuration file in multiple dimensions, and also extracts the extra dependencies and local environment related dependencies information. 

\textbf{PyPI API.} PyPI provides the "GET /pypi/<project\_name>/json" API, which could return the metadata about the latest release of the project and all releases infomation. After getting the release list, we use the "GET /pypi/<project\_name>/<version>/json" API to get the metadata information for each specific version. The metadata is a json containing basic information, dependency information and file download links. Although the API approach can simply get dependencies including extra dependency and local environment related dependency, we found that 10 percent(\textbf{need to check the number}) of the releases could not get the correct direct dependencies by the API alone. So we also need other methods to help reduce mistakes. \loancold{Introduce the so-called "other methods" right now, or readers are interrupted by this sentence.}

%需要加百分比统计吗
%需要加文件结构图吗
\begin{figure}
\centering
    \begin{subfigure}[b]{0.45\textwidth}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
pkg-0.0.1.tar.gz
--mod1
----__init__.py
--mod2.py
--setup.py
--pkg.egg-info
----PKG-INFO
----requires.txt
----SOURCES.txt
----top_level.txt
----entry_points.txt
----dependency_links.txt
\end{minted}
\caption{source package file format \xingyu{ replace by a real package }}
\label{fileformat:sdist}
\end{subfigure}

\centering
\begin{subfigure}[b]{0.45\textwidth}
\vspace{10pt}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
pkg-0.0.1-py3-none-any.whl
--mod1
----__init__.py
--mod2.py
--pkg-0.0.1.dist-info
----METADATA
----RECORD
----WHEEL
----top_level.txt
----LICENSE
\end{minted}
\caption{binary package file format \xingyu{replace by a real package}}  
\end{subfigure}%

\label{fileformat:wheel}
\caption{different file formats}
\label{fig:file format}
\vspace{-16pt}
\end{figure}

\label{chapt:metadata file}
\textbf{Metadata file.} Due to historical reasons, there are different formats of files on PyPI, which greatly increases the difficulty of extracting dependency information. Fortunately, we found that most of the files contain a folder with metadata information in it. For example, \cref{fig:file format} shows the file structure of two different formats of compressed packages. \cref{fileformat:sdist} shows the file structure of the tar.gz format, which typically contains the setup.py file and a pkg.egg-info folder. The setup.py file is the build script for the release, and the files in the pkg.egg-info folder are the files generated during the build process. The requirements.txt file records the direct dependency information, the PKG-INFO file records the metadata of the release, and the sources.txt file records all the pathes of the file. The whl package file format is very different from the tar.gz file. Since pip no longer compiles for the whl package, there is no setup.py script. In addition, the metadata of the whl package is stored in the dist-info folder. It does not have a dedicated requirement.txt file to store all dependency information, but it stores in the require\_dist field in the METADATA file. So, we need to parse the dependency information from the metadata files in different formats and convert them into a uniform format.However, not all source files have metadata files, so there is another way to get direct dependencies.

%需要加伪代码吗？
\label{chapt2:setup.py}
\textbf{Setup.py.} For source packages without metadata files, we use the setup.py installation script to get direct dependencies. First we will try to compile and run the install script to generate the metadata file, and then use the method referred in \cref{chapt:metadata file}. However, due to the python version and the local installer version, some packages will fail to build. So we use the hook function, hook setup function, to get the install\_require and extra\_require parameters in it. More specifically, we embed a fake setup function in the setuptools module, so that the script file uses the function we embedded when running the setup function. In the fake setup.py we first use the attr.get method to get the extra\_require and install\_require parameters, with them then we construct the direct dependency information in the uniform format we defined earlier. 

By using the above multi-dimensional dependency extraction methods, we are able to obtain a more accurate and universal dataset fastly.

\xingyu { Add Dependency Resolution. How to get transitive dependencies? }

\xingyu { Evaluation }


==> backups/module_path_semantic_identificat.tex <==
\section{Module path semantic identification}
\label{chapt:tech2}
This section we introduce how we recognize module path from different formats with our Module path semantic identification technique.

\begin{figure}
\centering
    \begin{subfigure}[b]{0.45\textwidth}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
setup(
    name = "pkg",
    version = "0.0.1",
    packages = ["mod1"],
    namespace_packages = ["mod1"],
    py_modules=["mod2"],
    }
)
\end{minted}
\caption{setup.py}
\label{example:setup}
\end{subfigure}

\centering
\begin{subfigure}[b]{0.45\textwidth}
\vspace{10pt}
\begin{minted}[fontsize=\footnotesize, linenos]{text}
pkg-0.0.1-py3-none-any.whl
--pkg-0.0.1-py3-nspkg.pth
--mod2.py
--pkg-0.0.1.dist-info
----METADATA
----RECORD
----WHEEL
----top_level.txt
----namespace_packages.txt
----LICENSE
\end{minted}
\caption{After installation}  
\end{subfigure}%
\label{example:diff after install}
\caption{different file structure}
\label{fig:example of install}
\vspace{-16pt}
\end{figure}
\subsection{Challenge}
Since packages on PyPi come in various formats, and the paths of the modules generated by different formats after installation via pip are not the same as the paths inside the compressed packages, which greatly increases the difficulty of parsing all the modules of a package. What's more, the installation behavior of pip relies on the installation script setup.py, which is an executable code file. Except for setup function, everyone has his way to write it. Most importantly, the logic of pip's behavior during installation is too complex, and even after getting the parameters related to the module path in setup.py, it is extremely difficult to translate the parameters into the paths after installation. 

For example, \cref{fileformat:sdist} is the source package file structure and \cref{example:setup.py} is the setup.py installation script. In the script, we define two modules, mod1 and mod2.py. However, \cref{example:diff after install} shows the modules after installation using pip. It has only mod2.py and replace mod1 with "pkg-0.0.1-py3-nspkg.pth", which means mod1 is a namespace\_package. So this example illustrates the complexity of pip installation behavior.

\subsection{related parameters and their behaviors}
\label{chapt:related parameters and their behaviors}
Based on our experimental research, we found that there are three parameters in the installation script related to the module path, including packages, namespace\_packages,py\_modules. 

\textbf{packages.} The packages parameter decides all the modules that are folders after installation. For example, if packages defines as $["mod1"]$, then the module paths will include "mod1/\_\_init\_\_.py"(mod1 itself) and all the submodules that are files("mod1/*.py"). It use "." to split module and its submodule. For example, if packages defines as $["mod1.submod"]$, then the module paths will include "mod1/submod/\_\_init\_\_.py" and "mod1/submod/*.py". In addition, the setuptools module also provides a "find\_packages" interface to automate the search for all modules and submodules in the current directory and its sub-directories. 

\textbf{namespace\_packages.} The namespace\_packages parameter decides all the namespace packages and it is a subset of the packages parameter\cite{pep420}. If this parameter is defined, the installation script will generate a file with the suffix nspkg.pth in the root directory and a namespace\_packages.txt file in the metadata folder. Besides, it will omit \_\_init\_\_.py file in its module if it has it. For example, \cref{example:setup} defines $["mod1"]$ as packages and namespace\_packages. Before installation, the project has mod1 with \_\_init\_\_.py in it and mod2.py. If we do not declare "mod1" as namespace package, the result is \cref{fileformat:wheel}. IF we declare. the result is \cref{example:diff after install} and it strip "mod1/\_\_init\_\_.py" and create a namespace\_packages.txt and a pkg-0.0.1-py-nspkg.pth.

\textbf{py\_modules.} The py\_modules parameter decides all the modules in the root directory. For example, \cref{example:setup} defines $["mod2"]$ as py\_modules, so the mod2.py will be considered in the modules after installation.

\subsection{parameters extraction}
Similar to the technique of extracting dependency information, we also extract the relevant fields from the metadata file and setup.py.
For binary files, the path extraction after installation is relatively simple, just read the RECORD file. This is because the RECORD file contains all the paths and hashes of the modules after the installation. However, it is more complicated to obtain the module paths for the source package, and it is necessary to extract the relevant parameters mentioned in \cref{chapt:related parameters and their behaviors} and then translate them through the algorithm\cref{alg:traslation}.

For those source packages that have metadata files, we extract the module path related information from the metadata files, which includes top\_level.txt, SOURCES.txt, namespace\_packages.txt. SOURCES.txt records the paths of all the files in the source package, including setup.py, which is not part of the module paths after installation. The top\_level.txt contains all the top-level module names. In \cref{fileformat:sdist} it reffers to mod1 and mod2, no matter how many sub-modules in the mod1. The namespace\_packages.txt records the names of the namespaces.

For those source packages that don't have metadata files, we use technique proposed in \cref{chapt2:setup.py} and extract packages, namespace\_packages, py\_modules parameters from setup.py. 
% \subsection{semantic translation to module paths}
% \cref{alg:traslation} shows our algorithm for translating parameters into module paths. Its input is project compressed file and its output is all module paths.


% It can be formally defined using the grammar below:
% \begin{equation}
%     form A = 
%     packages = \[\]
% \end{equation}


